Mark My Words: Analyzing and Evaluating Language Model Watermarks

The capabilities of large language models have grown significantly in recent years and so too have concerns about their misuse. It is important to be able to distinguish machine-generated text from human-authored content. Prior works have proposed numerous schemes to watermark text, which would benefit from a systematic evaluation framework. This work focuses on LLM output watermarking techniques - as opposed to image or model watermarks - and proposes Mark My Words, a comprehensive benchmark for them under different natural language tasks. We focus on three main metrics: quality, size (i.e., the number of tokens needed to detect a watermark), and tamper resistance (i.e., the ability to detect a watermark after perturbing marked text). Current watermarking techniques are nearly practical enough for real-world use: Kirchenbauer et al. [33]'s scheme can watermark models like Llama 2 7B-chat or Mistral-7B-Instruct with no perceivable loss in quality on natural language tasks, the watermark can be detected with fewer than 100 tokens, and their scheme offers good tamper resistance to simple perturbations. However, they struggle to efficiently watermark code generations. We publicly release our benchmark (https://github.com/wagner-group/MarkMyWords).

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We describe limitations in~\cref{ssec:discussion:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discuss societal impacts of our work in~\cref{app:societal-impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We include them in~\cref{app:ssec:pseudorandom-proofs}.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{We include them in~\cref{app:ssec:pseudorandom-proofs}.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We open-sourced the benchmark code at \url{https://github.com/wagner-group/MarkMyWords}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We did not perform training, but we specify watermarking hyperparmeters in~\cref{ssec:eval_aggregate}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report error bars for our main figure (\cref{fig:aggregate}). We discuss variance of each metric in~\cref{app:ssec:variance}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We include this in~\cref{sec:results}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the open-source large language models we use~\citep{llama3,jiang2023mistral}.}
  \item Did you mention the license of the assets?
    \answerYes{We mention the licenses of the open-source large language models in the references section~\cite{llama3,jiang2023mistral}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The new assets consist of our benchmark code, which is open-sourced at \url{https://github.com/wagner-group/MarkMyWords}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We did not curate data from any people.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We are not curating any data with personally identifiable information or offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects.}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> dataset_card.tex <==
\section{Datasheet}

Our primary contribution is our benchmark and its results. However, we do use a new dataset of inputs for evaluation, based on three tasks: book reports, story generation, and fake news. These do not have labeled outputs, as we care about the quality of generation relative to the original LLM, not in absolute terms. Below, we describe this dataset using the datasheets for datasets format~\cite{gebru2021datasheets}.

\datasheetsection{Motivation For Datasheet Creation}


\begin{datasheetitem}{For what purpose was the dataset created? \normalfont Was there a specific task in mind? Was there a specific gap that needed to be filled? Please provide a description.}
These tasks we chosen to be representative of potential misuse of LLMs.
They represent scenarios in which LLM could be abused 
and thus in which watermarking would be useful.
Up until this point, there was no common ground to evaluate watermarking schemes, and we introduce this dataset to fill that gap.
% More details are provided in~\cref{sec:experiments}.
\end{datasheetitem}


\begin{datasheetitem}{Who created the dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organization)?}

This dataset was created by Julien Piet, Chawin Sitawarin, Vivian Fang, Norman Mu and David Wagner. All creators are affiliated with the University of California, Berkeley.
    
\end{datasheetitem}

\begin{datasheetitem}{Who funded the dataset creation? \normalfont If there is an associated grant, please provide the name of the grantor and the grant name and number.}

The dataset creation was funded by the National Science Foundation, the KACST-UCB Joint Center on Cybersecurity, C3.ai DTI, Open Philanthropy, and Google. 

\end{datasheetitem}


\datasheetsection{Datasheet Composition}

\begin{datasheetitem}{What do the instances that comprise the dataset represent (e.g., documents, photos, people, countries)? \normalfont Are there multiple types of instances (e.g., movies, users, and ratings; people and interactions between them; nodes and edges)? Please provide a description.}

The instances are LLM prompts for the three tasks:
\begin{enumerate}[leftmargin=*,noitemsep,label=\textbf{(\arabic*)}]
    \item \textbf{Book reports.} Generate a report of a well-known book.
    \item \textbf{Story generation.} Generate a short story, with a specific tone (e.g., funny, sad, suspenseful) and topic (e.g., ``three strangers that win a getaway vacation'').
    \item \textbf{Fake news.} Generate a news story about two political figures meeting at an event.
\end{enumerate}
    
\end{datasheetitem}


\begin{datasheetitem}{How many instances are there in total (of each type, if appropriate)?}

There are 296 instances: 100 book report generation tasks, 96 story generation tasks, and 100 fake news generation tasks. 
    
\end{datasheetitem}
    
\begin{datasheetitem}{Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set? \normalfont If the dataset is a sample, then what is the larger set? Is the sample representative of the larger set (e.g., geographic coverage)? If so, please describe how this representativeness was validated/verified. If it is not representative of the larger set, please describe why not (e.g., to cover a more diverse range of instances, because instances were withheld or unavailable).}
Each instance is an example task, and the dataset could be made larger by including other examples (e.g., more books to review). However, this comes at the expense of increasing the runtime of our benchmark.
\end{datasheetitem}
\begin{datasheetitem}{What data does each instance consist of? \normalfont “Raw” data (e.g., unprocessed text or images) or features? In either case, please provide a description.}
Each instance consisits of a string of text consisting of the LLM input prompt and system prompt.
\end{datasheetitem}
\begin{datasheetitem}{Is there a label or target associated with each instance? \normalfont If so, please provide a description.}
There are no labels for this dataset.
\end{datasheetitem}
\begin{datasheetitem}{Is any information missing from individual instances? \normalfont If so, please provide a description, explaining why this information is missing (e.g., because it was unavailable). This does not include intentionally removed information, but might include, e.g., redacted text.}
No information is missing from individual instances.
\end{datasheetitem}
\begin{datasheetitem}{Are relationships between individual instances made explicit (e.g., users’ movie ratings, social network links)? \normalfont If so, please describe how these relationships are made explicit.}
N/A.
\end{datasheetitem}
\begin{datasheetitem}{Are there recommended data splits(e.g., training, development/validation, testing)? \normalfont If so, please provide a description of these splits, explaining the rationale behind them.}
This dataset is not meant for training. It is intended to be used during inference time.
\end{datasheetitem}
\begin{datasheetitem}{Are there any errors, sources of noise, or redundancies in the dataset? \normalfont If so, please provide a description.}
None.
\end{datasheetitem}
\begin{datasheetitem}{Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g., websites, tweets, other datasets)? \normalfont If it links to or relies on external resources, a) are there guarantees that they will exist, and remain constant, over time; b) are there official archival versions of the complete dataset (i.e., including the external resources as they existed at the time the dataset was created); c) are there any restrictions (e.g., licenses, fees) associated with any of the external resources that might apply to a dataset consumer? Please provide descriptions of all external resources and any restrictions associated with them, as well as links or other access points, as appropriate.}
This dataset is self-contained.
\end{datasheetitem}
\begin{datasheetitem}{Does the dataset contain data that might be considered confidential (e.g., data that is protected by legal privilege or by doctor-patient confidentiality, data that includes the content of individuals’ non-public communications)? \normalfont If so, please provide a description.}
No.
\end{datasheetitem}
\begin{datasheetitem}{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety? \normalfont If so, please describe why.}
Some prompts for story or fake news generation may contain moderately inappropriate or offensive language, but we do not expect this to be the normal case.
\end{datasheetitem}
\begin{datasheetitem}{Does the dataset identify any subpopulations (e.g., by age, gender)? \normalfont If so, please describe how these subpopulations are identified and provide a description of their respective distributions within the dataset.}
No.
\end{datasheetitem}
\begin{datasheetitem}{Is it possible to identify individuals (i.e., one or more natural persons), either directly or indirectly (i.e., in combination with other data) from the dataset? \normalfont If so, please describe how.}
No.
\end{datasheetitem}
\begin{datasheetitem}{Does the dataset contain data that might be considered sensitive in anyway (e.g., data that reveals race or ethnic origins, sexual orientations, religious beliefs, political opinions or union memberships, or locations; financial or health data; biometric or genetic data; forms of government identification, such as social security numbers; criminal history)? \normalfont If so, please provide a description.}
No.
\end{datasheetitem}
\datasheetsection{Collection Process}	
\begin{datasheetitem}{How was the data associated with each instance acquired? \normalfont Was the data directly observable (e.g., raw text, movie ratings), reported by subjects (e.g., survey responses), or indirectly inferred/derived from other data (e.g., part-of-speech tags, model-based guesses for age or language)? If the data was reported by subjects or indirectly inferred/derived from other data, was the data validated/verified? If so, please describe how.}
The dataset was handwritten by the dataset creators.

\end{datasheetitem}
\begin{datasheetitem}{What mechanisms or procedures were used to collect the data (e.g., hardware apparatuses or sensors, manual human curation, software programs, software APIs)? \normalfont How were these mechanisms or procedures validated?}
N/A.
\end{datasheetitem}
\begin{datasheetitem}{If the dataset is a sample from a larger set, what was the sampling strategy (e.g., deterministic, probabilistic with specific sampling probabilities)?}
N/A.
\end{datasheetitem}
\begin{datasheetitem}{Who was involved in the data collection process (e.g., students, crowdworkers, contractors) and how were they compensated (e.g., how much were crowdworkers paid)?}
The dataset creators (authors of this paper) were involved in the creation process.
\end{datasheetitem}
\begin{datasheetitem}{Over what timeframe was the data collected? \normalfont Does this timeframe match the creation timeframe of the data associated with the instances (e.g., recent crawl of old news articles)? If not, please describe the timeframe in which the data associated with the instances was created.}
N/A.
\end{datasheetitem}
\begin{datasheetitem}{Were any ethical review processes conducted (e.g., by an institutional review board)? \normalfont If so, please provide a description of these review processes, including the outcomes, as well as a link or other access point to any supporting documentation.}
N/A.
\end{datasheetitem}
\datasheetsection{Preprocessing/cleaning/labeling}	
\begin{datasheetitem}{Was any preprocessing/cleaning/labeling of the data done (e.g., discretization or bucketing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)? \normalfont If so, please provide a description. If not, you may skip the remaining questions in this section.}
None.
\end{datasheetitem}
\begin{datasheetitem}{Was the “raw” data saved in addition to the preprocessed/cleaned/labeled data (e.g., to support unanticipated future uses)? \normalfont If so, please provide a link or other access point to the “raw” data.}
N/A.
\end{datasheetitem}
\begin{datasheetitem}{Is the software that was used to preprocess/clean/label the data available? \normalfont If so, please provide a link or other access point.}
N/A.
\end{datasheetitem}
\begin{datasheetitem}{Any other comments?}
None.
\end{datasheetitem}

\datasheetsection{Uses}	
\begin{datasheetitem}{Has the dataset been used for any tasks already? \normalfont If so, please provide a description.}
Yes, the dataset has been used to evaluate both existing and new symmetric-key watermarking schemes.
\end{datasheetitem}
\begin{datasheetitem}{Is there a repository that links to any or all papers or systems that use the dataset? \normalfont If so, please provide a link or other access point.}
We keep a running list here: \url{https://github.com/wagner-group/MarkMyWords/blob/main/run/watermark_specs}.
\end{datasheetitem}
\begin{datasheetitem}{What (other) tasks could the dataset be used for?}
This dataset could be used in other benchmarks for evaluating watermarks that need natural language generation tasks.
\end{datasheetitem}
\begin{datasheetitem}{Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses? \normalfont For example, is there anything that a dataset consumer might need to know to avoid uses that could result in unfair treatment of individuals or groups (e.g., stereotyping, quality of service issues) or other risks or harms (e.g., legal risks, financial harms)? If so, please provide a description. Is there anything a dataset consumer could do to mitigate these risks or harms?}
No.
\end{datasheetitem}
\begin{datasheetitem}{Are there tasks for which the dataset should not be used? \normalfont If so, please provide a description.}
The dataset should strictly be used for evaluation. That is, the tasks should not be fed to language models to enable their misuse (e.g., publishing the fake news stories the language model generates).
\end{datasheetitem}
\datasheetsection{Distribution}	
\begin{datasheetitem}{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created? \normalfont If so, please provide a description.}

Yes, the dataset is publicly available on the internet.
\end{datasheetitem}
\begin{datasheetitem}{How will the dataset will be distributed (e.g., tarball on website, API, GitHub)? \normalfont Does the dataset have a digital object identifier (DOI)?}
The dataset is available as part of the benchmark at \mylink{https://github.com/wagner-group/MarkMyWords}.
The dataset itself is located at \url{https://huggingface.co/datasets/wagner-group/MarkMyWords-tasks}.
\end{datasheetitem}
\begin{datasheetitem}{When will the dataset be distributed?}
The dataset has been released on December 1st, 2023.
\end{datasheetitem}
\begin{datasheetitem}{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms o fuse (ToU)? \normalfont If so, please describe this license and/or ToU, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms or ToU, as well as any fees associated with these restrictions.}
We are licensing the dataset under a CC-BY license and the benchmark code under an Apache 2.0 license.
\end{datasheetitem}
\begin{datasheetitem}{Have any third parties imposed IP-based or other restrictions on the data associated with the instances? \normalfont If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms, as well as any fees associated with these restrictions.}
Unknown to the authors of the dataset.
\end{datasheetitem}
\begin{datasheetitem}{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances? \normalfont If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any supporting documentation.}
No.
\end{datasheetitem}
\datasheetsection{Maintenance}	
\begin{datasheetitem}{Who will be supporting/hosting/maintaining the dataset?}
The authors will support the dataset. It is hosted on GitHub.
\end{datasheetitem}
\begin{datasheetitem}{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}
The lead author, Julien Piet, can be contacted at \url{https://people.eecs.berkeley.edu/~julien.piet/}.
\end{datasheetitem}
\begin{datasheetitem}{Is there an erratum? \normalfont If so, please provide a link or other access point.}
No.
\end{datasheetitem}
\begin{datasheetitem}{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances)? \normalfont If so, please describe how often, by whom, and how updates will be communicated to dataset consumers (e.g., mailing list, GitHub)?}
There are no plans to update the dataset, but if errors need to be corrected, updates will be issued on GitHub.
\end{datasheetitem}
\begin{datasheetitem}{Will older versions of the dataset continue to be supported/hosted/maintained? \normalfont If so, please describe how. If not, please describe how its obsolescence will be communicated to dataset consumers.}
Yes, they will continue to be hosted on GitHub.
\end{datasheetitem}
\begin{datasheetitem}{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so? \normalfont If so, please provide a description. Will these contributions be validated/verified? If so, please describe how. If not, why not? Is there a process for communicating/distributing these contributions to dataset consumers? If so, please provide a description.}
Contributors can fork the GitHub repository and submit a pull request.
\end{datasheetitem}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> param_tuning.tex <==
\section{Parameter tuning}
\label{app:param-tuning}
\ifappendixonly
We now elaborate on how we arrived at the parameter suggestions in Table 3 of the main paper.
\else
We now elaborate on how we arrived at the parameter suggestions in~\cref{table:parameter-effects}.
\fi

\smallskip\noindent{\bf Window size.} 
Increasing the window size increases quality, but also increases the watermark size and decreases robustness.
We recommend using a window size of 1 to 3; larger window sizes do not further improve quality.

\smallskip\noindent{\bf Min hash.} 
At a window size of 3, the min hash increases both tamper resistance and size by 33\%, compared to a sliding window.
We recommend using a simple sliding window.

\smallskip\noindent{\bf Skip probability.} 
We recommending setting the skip probability at 0.05 
for indistinguishable schemes (exponential, binary, inverse transform) 
using text-dependent randomness, 
as this adds non determinism to their outputs. 
This also provides slightly better quality than a skip probability of 0.

\smallskip\noindent\textbf{Bias.} 
For distribution-shift, the bias ($\delta$) is a critical parameter
that has a large impact on quality, size, and tamper resistance.
\cref{bias-fig} visualizes its impact.
We suggest choosing $\delta$ based on the most common
temperature that the model is likely to be used with.
In all cases, only values of $\delta \geq 2$ yield efficient schemes.

\smallskip\noindent{\bf Green list size.}
Our early experiments showed that changing the green list size ($\gamma$) from 
0.5 only negatively impacts the watermark in all three metrics.
Therefore we fixed $\gamma$ to 0.5 for our experiments and suggest practitioners do the same. 

\smallskip\noindent{\bf Fixed randomness.} 
We recommend using a key length $L$ of 4.
Smaller values are detrimental to quality, but for $L \geq 4$ quality remains mostly the same, while larger values are worse for tamper resistance and size (\cref{keylen-fig}).

==> prior_reviews.tex <==
\section{Prior submission}

This work was previously submitted to the Conference on Language Models (COLM 2024). Overall, reviewers praised the work for its thoroughness, usefulness of the metrics, reproducibility, and valuable insights. They critiqued the original choice of using Llama 2 to rate its own generations, the lack of an evaluation on low-entropy tasks, and suggested introducing MAUVE as an auxiliary quality metric. We withdrew the paper to work on these points, and made the following changes:
\begin{itemize}
    \item Switch to Llama 3 for rating, to avoid self-bias in using Llama 2 to rate its own generations~\cite{xu2024perils}.
    \item Added the MAUVE score as an additional metric, to validate our results.
    \item Evaluated the optimal watermarks on two low entropy tasks --- paraphrasing and translation.
    \item Evaluated the optimal watermarks on code generations
\end{itemize}

==> reprod.tex <==
\section{Reproducibility statement}
\label{s:reprod-statement}
\subsection{Implementation}
% \subsection{Benchmark Implementation}
% \label{ss:benchmark-imple}
We implemented the \benchmarkname{} benchmark in Python using the \texttt{transformers} library~\citep{wolf_transformers_2020} to implement models and watermarks.
%
In general, the run times of the watermarked models are comparable to those of base models.
%
We rely on the 7B-parameter version of Llama 2 chat both for generation and rating.
%
We chose this model for its high quality and because its output distribution, like other modern models, has low entropy.
We've noticed newer language models are more certain of their next-token predictions, i.e., have lower entropy in their output distribution,
which makes watermarking more difficult. Thus, using a low-entropy model makes for a more realistic 
evaluation of a watermark scheme's performance. 
%
This version of the Llama 2 model is known for often refusing to generate content---we 
altered the system prompt to avoid this issue, especially for the fake news task.

%Users can choose whether to sample a new secret watermarking key for each generation or not.
%
%We enable this in our experiments, but practitioners can deactivate it in order to evaluate a model's performance for a specific secret key, for instance when evaluating a public scheme.

Our code for the \benchmarkname{} benchmark has been made public.\footnote{\mylink{https://anonymous.4open.science/r/MarkMyWords}}
%
It supports many language models, and allows passing custom watermarking schemes for evaluating new solutions. 
%Anyone can run it, either to compare new watermarking schemes to the ones presented in the paper, or to find the best hyper-parameter 
%selection for another language model. 
%
% We hope that future proposals of watermark schemes will include an evaluation with this benchmark.
We designed \benchmarkname{} with the goal of making future proposals of watermark schemes straightforward to evaluate.

\subsection{Efficiency}
%
In order to speed up computation, we wrote custom implementations directly in CUDA of some of the watermarking schemes:
\begin{itemize}[leftmargin=\itemlm,nosep]
    \item \textbf{Hash function.} The exponential sampling scheme relies on computing the hash of many elements. Our CUDA implementation allows this to be done in parallel.
    \item \textbf{Edit distance.} The edit distance is computed with every possible key offset; our code implements this in parallel.
\end{itemize}
% Additionally, for empirical verification of edit scores, since we use a $t$-test~\cite{kuditipudi_robust_2023}, we need to compute test statistic 100 times under the null hypothesis to derive an empirical $p$-value.
% %
% This is done by replacing the randomness used at generation time by fresh random 
% values.
% Doing so for each detection is inefficient.
% %
% Instead, for edit scores, we pre-compute the test statistic under the null hypothesis 200 times and then sample 100 random values of this statistic every time we want to verify a watermark.
% \chawin{I'm a bit confused by this part.}
% %
% This means we only need to run the expensive computation once.
% %
% Empirically, we did not see a change in detection accuracy when doing so. 
